Electrostatic interactions in atomistic and machine-learned potentials for polar materials

Long-range electrostatic interactions critically affect polar materials. However, state-of-the-art atomistic potentials, such as neural networks or Gaussian approximation potentials employed in large-scale simulations, often neglect the role of these long-range electrostatic interactions. This study introduces a novel model derived from first principles to evaluate the contribution of long-range electrostatic interactions to total energies, forces, and stresses. The model is designed to integrate seamlessly with existing short-range force fields without further first-principles calculations or retraining. The approach relies solely on physical observables, like the dielectric tensor and Born effective charges, that can be consistently calculated from first principles. We demonstrate that the model reproduces critical features, such as the LO-TO splitting and the long-wavelength phonon dispersions of polar materials, with benchmark results on the cubic phase of barium titanate (BaTiO$_3$).

==> src/polarizability.tex <==

\section{The polarizability contribution to energy}

The only contribution of energy accounted in \eqname~\eqref{eq:energy} is from the dipole generated by lattice displacements.
However, there is another contribution to the total energy, which is the one that raises from an external electric field on the electronic suscieptibility.

\begin{equation}
  {\mathcal E}^{(el)} = -\frac 12 \sum_{\alpha\beta} E_\alpha \chi_{\alpha\beta} E_\beta
  \label{eq:energy:el}
\end{equation}

This means that, in presence of an external electric field, the electronic medium that envelop the full system of ions produces a dipole moment itself. This also holds for the electric field produced by the ionic displacements, thus it give rise to a force. The electric field in \eqname~\eqref{eq:energy:el} is the macroscopic electric field generated inside the material from the ionic displacements.

\textbf{\color{red}
TODO: Think who is the electric field. THe paper of Cochran and Cowley takes an electric field which is a constant vector for displacements along $\Gamma$ which is exactly what we are doing.
Probably this full treatment is completely wrong, what is actually correct is to use the fact that the production of a dipole generates only a uniform electric field inside the material. Probably this simplifies a lot the equations as there is no more the need to specify the actual location of the dipoles.}


==> src/stress_old.tex <==

\section{Stress tensor}

We have energy and forces, we could also get the long-range stress contribution:
\begin{equation}
\sigma_{\alpha\beta} = -\frac {1}{\Omega} \frac{d \mathcal{E}}{d\varepsilon_{\alpha\beta}}
\end{equation}

where $\bsigma$ is the stress tensor, $\boldsymbol{\varepsilon}$ the strain tensor and $\Omega$ the unit cell volume. We recall how the atomic position changes after a uniform strain:
\begin{equation}
R_{i\alpha}' = R_{i\alpha} + \sum_{\beta}\varepsilon_{\alpha\beta} R_{i\beta}
\end{equation}

If we transform the total energy according to a strain, we get:
\begin{equation}
\mathcal{E}(\boldsymbol{\varepsilon}) = -\sum_{i\alpha\beta\gamma}(\delta_{\alpha\gamma} + \varepsilon_{\alpha\gamma})(R_{i\gamma} - {\Rcal}_{i\gamma}) Z_{i\beta\alpha} E_{i\beta}(\boldsymbol{\varepsilon})
\end{equation}

So this derivative has two contributions, one comes from the change on the dipole following the strain, the other in the change of the electric field as all the other dipoles in the system changes.
In particular:
\begin{align}
\sigma_{\alpha\beta} = \frac {1}{\Omega}&\bigg[\frac 12 \sum_{i\gamma}(R_{i\beta} - \Rcal_{i\beta})Z_{i\gamma\alpha}E_{i\gamma} +  \nonumber \\
& + \frac 1 2 \sum_{i\gamma}(R_{i\alpha} - \Rcal_{i\alpha})Z_{i\gamma\beta}E_{i\gamma} +  \nonumber \\
& + \sum_{i\gamma\delta}(R_{i\gamma} - \Rcal_{i\gamma})Z_{i\delta\gamma}\frac{d E_{i\delta}}{d\varepsilon_{\alpha\beta}}\bigg]
\label{eq:stress}
\end{align}

where the first two terms have been symmetrized with respect to $\alpha\leftrightarrow\beta$, to match the constrain of symmetric deformation of the strain tensor.
So the most complex term is the last one. The electric field depends on the strain as the dipoles that generate it depend, as well as the position operators inside it.
\begin{equation}
\bE_{i}(\bvareps) = \sum_{j\neq i}\frac{q_j}{4\pi\varepsilon_0} \frac{\dielectric^{-1}(\identity + \bvareps)(\br_i - \tilde\bR_j(\bvareps))}{\left|(\identity + \bvareps)(\br_i - \tilde\bR_j(\bvareps))\right|^3} 
\end{equation}
where $\identity$ is the identity 3x3 matrix and $\br_i$ the position of the dipole of the $i$-th atom, w
$$
\br_i = \frac{\bR_i + \bRcal_i}{2}
$$
\begin{widetext}
\begin{align}
\frac{dE_\mu}{d\varepsilon_{\alpha\beta}} = \sum_{j\neq i,\nu\lambda} \frac{q_j\ldielectric^{-1}_{\mu\nu}}{4\pi\varepsilon_0} &  \left[\frac{\delta_{\lambda\nu}}{\left|\br_i - \tilde\bR_j\right|^3} - \frac{3\left(r_{i\lambda} - \tilde R_{j\lambda}\right)\left(r_{i\nu} - \tilde R_{j\nu}\right)}{\left|\br_i - \tilde\bR_j\right|^5} \right]\cdot\nonumber \\
& \cdot \left[\frac 12\delta_{\lambda\alpha}(r_{i\beta} - \tilde R_{j\beta}) + \frac 12\delta_{\lambda\beta}(r_{i\alpha} - \tilde R_{j\alpha})
-\frac{\partial \tilde R_{j\lambda}}{\partial\varepsilon_{\alpha\beta}}
\right]\label{eq:field:stress}
\end{align}
\end{widetext}

We kept the explicit derivative of $\tilde R_{j\lambda}$ with respect to the strain. This is because this derivative is tricky, as it does not change as a normal vector. In particular, when we strain \eqname~\eqref{eq:rtilde}, we get:
\begin{align}
\tilde R_{i\alpha\pm}(\bvareps) &= \sum_\beta (\delta_{\alpha\beta} + \varepsilon_{\alpha\beta})\frac{R_{i\beta} + \Rcal_{i\beta}}{2} +\nonumber \\
&\pm \frac 1 q \sum_{\beta\gamma} Z_{i\alpha\beta}(\delta_{\beta\gamma} + \varepsilon_{\beta\gamma})(R_{i\gamma} - \Rcal_{i\gamma}) 
\end{align}

Unfortunately, the $\identity + \bvareps$ tensor not always commutes with the effective charge tensor, therefore $\tilde R_{i\alpha\pm}$ does not strain as a normal vector. However, we can add and subtract a contribution to have two different part of the tensor, one that strains as a normal vector, and the other that contain the deviation to the standard strain.

\begin{align}
\tilde R_{i\alpha\pm}(\bvareps) &= \sum_\beta (\delta_{\alpha\beta} + \varepsilon_{\alpha\beta})\frac{R_{i\beta} + \Rcal_{i\beta}}{2} +\nonumber \\
&\pm\frac 1 q \sum_{\beta\gamma}(\delta_{\alpha\gamma} + \varepsilon_{\alpha\gamma}) Z_{i\gamma\beta}(R_{i\beta} - \Rcal_{i\beta}) + \nonumber \\ 
&\mp \frac 1 q \sum_{\beta\gamma}(\delta_{\alpha\gamma} + \varepsilon_{\alpha\gamma}) Z_{i\gamma\beta}(R_{i\beta} - \Rcal_{i\beta}) + \nonumber \\
& \pm \frac 1 q \sum_{\beta\gamma} Z_{i\alpha\beta}(\delta_{\beta\gamma} + \varepsilon_{\beta\gamma})(R_{i\gamma} - \Rcal_{i\gamma})
\end{align}

The last term is essentially the commutator between the effective charge and the strain tensor and it is the one to be accounted for in the explicit derivative of the $\tilde R_{j\lambda}$ inside \eqname~\eqref{eq:field:stress}.


\begin{align}
\frac{\partial \tilde R_{i\lambda\pm}}{\partial \varepsilon_{\alpha\beta}}  = &\mp \frac 1 {q} \sum_\gamma \frac{\delta_{\alpha\lambda}Z_{i\beta\gamma} + \delta_{\beta\lambda}Z_{i\alpha\gamma}}{2}(R_{i\gamma} - \Rcal_{i\gamma}) + \nonumber \\
& \pm \frac 1 q \sum_\gamma \frac{Z_{i\lambda\alpha}(R_{i\beta} - \Rcal_{i\beta}) + Z_{i\lambda\beta}(R_{i\alpha} - \Rcal_{i\alpha})}{2}
\label{eq:commutator}
\end{align}


This concludes the derivation of the stress tensor, by substituting \eqname~\eqref{eq:commutator} into \eqname~\eqref{eq:field:stress} into \eqname~\eqref{eq:stress}.

